Quantized Frank-Wolfe: Faster Optimization, Lower Communication, and Projection Free

How can we efficiently mitigate the overhead of gradient communications in distributed optimization? This problem is at the heart of training scalable machine learning models and has been mainly studied in the unconstrained setting. In this paper, we propose Quantized-Frank-Wolfe (QFW), the first projection-free and communication-efficient algorithm for solving constrained optimization problems at scale. We consider both convex and non-convex objective functions, expressed as a finite-sum or more generally a stochastic optimization problem, and provide strong theoretical guarantees on the convergence rate of QFW. This is accomplished by proposing novel quantization schemes that efficiently compress gradients while controlling the noise variance introduced during this process. Finally, we empirically validate the efficiency of QFW in terms of communication and the quality of returned solution against natural baselines.

==> app_finite.tex <==
%!TEX root = main.tex
\section{Analysis on Finite-Sum Optimization}
\label{app:finite}
In this section, we will analyze the finite-sum problem defined in 
\eqref{finite_sum_problem}. Recall that we assume that there are $N$ functions 
and $M$ workers in total, and each worker $m$ has access to $n=N/M$ functions 
$f_{m,i}$ for $i \in [n]$. The major 
difference with the stochastic setting is that we can use a more aggressive 
variance reduction for communicating quantized gradients. More 
specifically, \citet{nguyen2017sarah,nguyen2017stochastic,nguyen2019optimal} 
developed the 
StochAstic Recursive grAdient algoritHm (SARAH), a stochastic recursive 
gradient update framework. 
Recently, \citet{fang2018spider} proposed  Stochastic 
Path-Integrated Differential Estimator (SPIDER) technique, a variant of SARAH, 
for unconstrained 
optimization in centralized settings. In this paper,  we properly generalize 
SPIDER to the constrained and distributed settings. 


To do so, we first consider the unquantized case. Let $p \in \mathbb{N}^+$ be a 
period parameter. At the 
beginning of each period, namely, \text{mod}$(t,p)=1$, each worker $m$, 
computes the average of all its local gradients and sends it to the master. 
Then, master calculates the average of the $M$ received signals and broadcasts 
it to all 
the workers. Then, the workers update their gradient estimation $\bar{g}_t$ as 
%%%
\begin{equation*}
\bar{g}_{t} = \frac{1}{Mn}\sum_{m=1}^M \sum_{i=1}^n \nabla 
f_{m,i}(x_t).
\end{equation*}

Note $\bar{g}_t$ is identical for all the workers. In the remaining iterations 
of 
that 
period, \emph{i.e.}, \text{mod}$(t,p)\neq 1$, each 
worker $m$ samples a set of local component functions, denoted as 
$\mathcal{S}_{t}^m$, of 
size $S$ uniformly at random, 
computes the average of these local gradients and sends it to master. Then, 
master calculates the average of the $M$ signals and broadcasts it to all 
the workers. The workers update their gradient estimation $g_t$ as
%and updates its local gradient estimate $g_{m,t}$ as follows:
\begin{equation*}
\bar{g}_{t} = \bar{g}_{t-1}+\frac{1}{MS}\sum_{m=1}^M\sum_{i 
	\in \mathcal{S}_{t}^m}[\nabla f_{m,i}(x_t)-\nabla 
f_{m,i}(x_{t-1})] .
\end{equation*}

So $\bar{g}_t$ is still identical for all the workers.
%
%To do so, let us define a period parameter $p \in \mathbb{N}^+$. 
%
%
%Each worker $m$ samples $S$ i.i.d. component functions 
%		uniformly at random, defines $\mathcal{S}_{t,m}$ to be the sample set, 	
%		and gets exact gradients $\nabla f_{m,i}(x_t), \nabla f_{m,i}(x_{t-1})$ 
%		for all $i \in \mathcal{S}_{t,m}$ 
%		\STATE Each worker pushes the quantization 
%		$\Phi_{1,t}\left({\sum_{i 
%				\in \mathcal{S}_{t,m}}\nabla f_{m,i}(x_t)-\nabla 
%			f_{m,i}(x_{t-1})}/{S}\right)$ 
%		to the master
%
%Similar to \cref{alg:dist_fw}, \cref{fig:workflow} describes the basic 
%workflow 
%of the proposed algorithm, too.
%%Here, the workflow of our proposed algorithm is similar to that of 
%%\cref{alg:dist_fw}. At each iteration, each worker sends the quantized 
%%version 
%%of some gradient information to the master. Then the master decodes the 
%%quantizations and calculates the average of them. Finally, the master 
%%broadcasts the quantized average to each worker, and each worker decodes it 
%%to 
%%update $x_t$ locally. 
%The major difference is that another kind of quantized gradient information is 
%communicated for the purpose of variance reduction. 
%
%
%Specifically, we adopt the 
%Stochastic Path-Integrated Differential Estimator (SPIDER) technique, which 
%was 
%first proposed in \citep{fang2018spider} for unconstrained non-convex 
%optimization problem in non-parallel setting.
%
%Suppose the objective function $f(x) = \frac{1}{N}\sum_{i=1}^N 
%f_i(x)$. In the 
%SPIDER technique, we 
%first set the period parameter $p \in \mathbb{N}^+$. If \text{mod}$(t,p)=1$, 
%we update
%\begin{equation*}
%g_t \gets \nabla f(x_t).
%\end{equation*}
%Otherwise, we sample $|\mathcal{S}_t|$ i.i.d. component functions uniformly, 
%where 
%$\mathcal{S}_t$ is the sample set. Then we update
%\begin{equation*}
%g_t \gets \frac{1}{|\mathcal{S}_t|} \sum_{i \in \mathcal{S}_t}[\nabla f_i(x_t) 
%- \nabla f_i(x_{t-1})] + g_{t-1}.
%\end{equation*}
%
%The vectors $g_t$'s are the gradient estimations which we will use in the 
%optimization algorithm, \emph{e.g.}, gradient descent or FW algorithm. 
%
%%We note that the SPIDER technique has a period $p$. 
%Note that at the beginning of each period, \emph{i.e.}, \text{mod}$(t,p)=1$, 
%we 
%start over and update $g_t$ by the exact gradient $\nabla f(x_t)$. In the rest 
%of the period, we use the previous estimation $g_{t-1}$ and newly sampled 
%gradients to provide new estimation. So the estimations within different 
%periods will not influence each other.
In order to incorporate quantization, each worker simply pushes the quantized 
version of the average gradients. Then the 
master decodes the quantizations, encodes the average of decoded 
signals in a quantized fashion, and broadcasts the quantization. Finally, 
each worker 
decodes the quantized signal and updates $x_t$ 
locally. 
%
%
%SPIDER into parallel algorithm with gradient 
%quantization, we need to ensure that each worker calculates the 
%corresponding $g_t$, and pushes it in a quantized manner. Then the 
%master decodes the quantizations, encodes the average of decoded 
%signals in a quantized fashion, and broadcasts the quantization. Finally, 
%each worker 
%decodes the quantized signals and updates $x_t$ 
%locally. 
%
The full description of our proposed \fAlg (F-QFW) algorithm is outlined 
in \cref{alg:finite_dist_fw}.

\begin{algorithm}[h]
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} constraint set $\constraint$, iteration 
		horizon $T$, number of workers $M$, initial 
		point $x_1 \in \constraint$, step sizes 
		$\eta_t$, period parameter $p$, sample size $S$
		\STATE {\bfseries Output:} $x_{T+1}$ %(for the convex setting) 
		or $x_o$, %(for the non-convex setting), 
		where $x_o$ is chosen from $\{x_1, x_2, 
		\cdots, x_T\}$ uniformly at random
		%$x_{T+1} \in \constraint$
		\FOR{$t=1$ {\bfseries to} $T$}
		\IF {\text{mod}$(t,p)=1$} 
		\STATE Each worker $m$ computes its local gradient 
		$g_t^m(x_t)=\frac{1}{n}\sum_{i=1}^n \nabla f_{m,i}(x_t)$
		\STATE Each worker $m$ encodes $g_t^m(x_t)$ as $\Phi_{1,t}(g_t^m(x_t))$ 
		and pushes it to the master
		\STATE Master decodes $\Phi_{1,t}(g_t^m(x_t))$ as 
		$\Phi_{1,t}^{\prime}(g_t^m(x_t))$
		\STATE Master computes the average gradient $\tilde{g}_t \gets 
		\frac{1}{M}\sum_{m=1}^M \Phi_{1,t}^{\prime}(g_t^m(x_t))$
		\STATE Master encodes $\tilde{g}_t$ as $\Phi_{2,t}(\tilde{g}_t)$, 
		and broadcasts it to all workers
		\STATE Workers decode
		$\Phi_{2,t}(\tilde{g}_t)$ as $\Phi_{2,t}^{\prime}(\tilde{g}_t)$ and 
		update $\bar{g}_t \gets \Phi_{2,t}^{\prime}(\tilde{g}_t)$
		\ELSE 
		\STATE Each worker $m$ at time $t$ samples $S$ component functions 
		uniformly at random called $\mathcal{S}_{t}^m$
		\STATE Each worker $m$ computes exact gradients $\nabla f_{m,i}(x_t), 
		\nabla f_{m,i}(x_{t-1})$ for all $i \in \mathcal{S}_{t}^m$ 
		\STATE Each worker $m$ encodes
		$\Phi_{1,t}(\frac{1}{S}{\sum_{i 
				\in \mathcal{S}_{t}^m}[\nabla f_{m,i}(x_t)-\nabla 
			f_{m,i}(x_{t-1})]})$ 
		and pushes to master
		\STATE Master decodes the signals 
		$\Phi_{1,t}(\frac{1}{S}{\sum_{i 
				\in \mathcal{S}_{t}^m}[\nabla f_{m,i}(x_t)-\nabla 
			f_{m,i}(x_{t-1})]})$
		\STATE Master computes $\tilde{g}_t \gets 
		\frac{1}{M}\sum_{m=1}^M \Phi_{1,t}^\prime 
		(\frac{1}{S}{\sum_{i 
				\in \mathcal{S}_{t}^m}[\nabla f_{m,i}(x_t)-\nabla 
			f_{m,i}(x_{t-1})]})$
		\STATE Master encodes $\tilde{g}_t$ as $\Phi_{2,t}(\tilde{g}_t)$, 
		and broadcasts all workers
		\STATE Workers decode
		$\Phi_{2,t}(\tilde{g}_t)$ as $\Phi_{2,t}^{\prime}(\tilde{g}_t)$ and 
		update $\bar{g}_t \gets \Phi_{2,t}^{\prime}(\tilde{g}_t)+\bar{g}_{t-1}$
		\ENDIF
		%\State The master encodes $\bar{g}_t \gets (1-\rho_t)\bar{g}_{t-1} + 
		%\rho_t\tilde{g}_t$ as $\phi(\bar{g}_t)$, and broadcast it to each 
		%worker
		%\State Each worker updates $x_{t+1}$ locally by $v_{t} \gets 
		%\argmin_{v \in \constraint} \langle v, \phi(\bar{g}_t) \rangle $ and 
		%$x_{t+1} \gets x_t + \eta_t(v_t-x_t)$
		\STATE Each worker updates $x_{t+1}$ locally by $x_{t+1} \gets 
		x_t 
		+ \eta_t(v_t-x_t)$ where $v_{t} \gets \argmin_{v 
			\in \constraint} \langle v, \bar{g}_t \rangle $
		\ENDFOR
		%		\STATE Output $x_{T+1}$ (for the convex setting) or $x_o$ (for 
		%the 
		%non-convex setting), where $x_o$ is chosen from $\{x_1, 
		%		x_2, \cdots, x_T\}$ uniformly at random
	\end{algorithmic}
	\caption{\fAlg (F-QFW)\label{alg:finite_dist_fw}}
\end{algorithm}

\textcolor{red}{We note that the more aggressive variance 
reduction technique, \emph{i.e.}, 
SPIDER, makes the noise caused by the quantization (rather than the noise from 
stochastic gradients) become the dominating variance. As a result, unlike \Alg, 
we can use finer quantization (\emph{e.g.}, Multi-Partition Quantization Scheme)
to achieve better convergence rate. We illustrate this effect in the following 
theoretical analysis as well as the numeric experiments.}

%Compared with \Alg, one advantage of \fAlg is 
%that we can use different quantization schemes $\{\Phi_{1,t}, \Phi_{2,t}\}$ at 
%different iterations $t$, which makes \cref{alg:finite_dist_fw} more flexible 
%in solving various optimization problems. \textcolor{red}{mr: the more 
%	aggressive variance reduction makes it possible to achieve better 
%	convergence 
%	rate by finer quantization, i.e., the noise caused by the quantization 
%	becomes 
%	the dominating variance} We will explore their effects empirically in our 
%	experiments.

%Another difference between \cref{alg:dist_fw,alg:finite_dist_fw}  
%Finally, note again that FW is very sensitive to  the accuracy of gradients in 
%order to converge. Nevertheless, we next give strong  theoretical guarantees 
%on 
%the 
%convergence rate of \fAlg for both convex and non-convex 
%settings while using quantized and local gradients distributed over $M$ 
%machines. 

%
%We note that the original SPIDER technique in \citep{fang2018spider} was not 
%applied on FW 
%algorithm or the parallel settings. Since 
%FW algorithm is extremely sensitive to the accuracy of gradients, it is an 
%interesting question whether SPIDER can help FW algorithm get good performance 
%when fed with quantized gradient information in parallel setting. This paper 
%gives a positive answer. We provide strong theoretical guarantees on the 
%convergence rate of \cref{alg:finite_dist_fw}, for both convex and non-convex 
%settings.

%We will show that \fAlg has good theoretical guarantees 
%(\cref{thm:finite_convex,thm:quantized_finite_distributed_nonconvex}) and 
%empirical performances (\cref{sec:experiments}). 

\subsection{Convex Optimization}
To analyze the convex case, we first make an assumption on the component 
functions.

\begin{assump}
	\label{assump_on_f_i_convex}
	The component functions $f_{m,i}$'s are convex, $L$-smooth on 
	$\constraint$, and uniformly bounded, i.e.,  $\sup_{x \in 
		\constraint}|f_{m,i}(x)| \leq M_0, \forall\ m \in [M], i \in [n]$.
\end{assump}
Since functions $f_{m,i}$ are all bounded and $L$-smooth on the compact 
constraint set $\constraint$, 
their gradients $\|\nabla f_{m,i}\|_\infty$ are also bounded on $\constraint$. 
Moreover, we only have a finite number of component functions 
$f_{m,i}$'s, thus, there will always be a uniform bound $G_\infty > 0$ on 
$\|\nabla 
f_{m,i}\|_\infty, \forall\ m \in [M], i \in [n]$. For 
simplicity of analysis, we assume an explicit upper bound $G_\infty$ in the 
following theorem. But this is a direct implication of the other assumptions.
\begin{mdframed}
	\begin{theorem}[Proof in \cref{app:thm_finite_convex}]
		\label{thm:finite_convex}
		Let us set $\eta_t=\frac{2}{p\lceil \frac{t}{p} \rceil }, p=\sqrt{n}, 
		S=\sqrt{n}$,  
		and apply  $s_{1,t}=(2^{z_{1,t}}-1)$-\mscheme 
		$\phi_{1,t}$, and  $s_{2,t}=(2^{z_{2,t}}-1)$-\mscheme $\phi_{2,t}$ as 
		$\Phi_{1,t}, \Phi_{2,t}$ in \cref{alg:finite_dist_fw} where 
		$z_{1,t}=\lceil\log_2[(\frac{pd^{1/2}S^{1/2}}{M^{1/2}})\lceil 
		\frac{t}{p} \rceil+1]\rceil, z_{2,t}=\lceil\log_2[ 
		pd^{1/2}S^{1/2}\lceil 
		\frac{t}{p} \rceil+1]\rceil$.
		Under \cref{assump_on_K,assump_on_f_i_convex}, and
		$\sup_{x \in \constraint}\|\nabla f_{m,i}(x)\|_\infty \leq G_\infty, 
		\forall\ m \in [M], i \in [n]$, and after $T$ 
		iterations, the output $x_{T+1} \in \constraint$  satisfies
		\begin{equation*}
		\expect[f(x_{T+1})]-f(x^*) \leq \frac{Q_0}{T},  
		\end{equation*}
		where  $Q_0=\max\{6pM_0, 3Q\}$, 
		$Q=4D(\sqrt{L^2D^2+2G_\infty^2}+LD)$, and $x^*$ 
		is a minimizer of $f$ on $\constraint$. %In other word, the output 
		%of \fAlg 
		%	is $\epsilon$-suboptimal with at most $\frac{Q_0}{\epsilon}$ 
		%rounds, 
		%	\emph{i.e.}, the LO (Linear-optimization Oracle) complexity is 
		%	$O(1/\epsilon)$. Also, the total IFO (Incremental First-order 
		%Oracle)
		%	complexity is $M[3\sqrt{n}-2]\frac{Q_0}{\epsilon} 
		%	=O(n/\epsilon)$. 
		
		%	Moreover, we only need at most about
		%	$d(M\lceil\log_2[(\frac{\sqrt{n}dT^2}{M})^{1/2}+1]\rceil+
		%	\lceil\log_2[(\sqrt{n}dT^2)^{1/2}+1]\rceil)+(M+1)(d+32)$
		%	 bits for communication per round.
	\end{theorem}
\end{mdframed}
%
%We note that if function $f_{m,i}$ is bounded and has $L$-Lipschitz continuous 
%gradient on the compact constraint set $\constraint$, 
%then $\|\nabla f_{m,i}\|_\infty$ is bounded on $\constraint$. 
%Since we have a finite number of component functions 
%$f_{m,i}$'s, there will always be a uniform bound of $\|\nabla 
%f_{m,i}\|_\infty \forall\ m \in [M], i \in [n]$ on $\constraint$. For 
%simplicity of analysis, we assume the explicit upper bound $G_\infty$ in the 
%theorem statement. But it is a direct implication of the other assumptions.

\cref{thm:finite_convex} indicates that in convex setting, if we 
use the recommended quantization schemes, then the output of 
\fAlg is 
$\epsilon$-suboptimal with at most $\frac{Q_0}{\epsilon}$ rounds, 
\emph{i.e.}, the Linear-optimization Oracle  (LO) complexity is 
$\mathcal{O}(\sqrt{n}/\epsilon)$. Also, the total Incremental First-order 
Oracle  (IFO) complexity is %$M[3\sqrt{n}-2]\frac{Q_0}{\epsilon} =
$[Mn+(p-1)\times M \times S \times 2] \times 
\frac{T}{p}=\mathcal{O}(n/\epsilon)$. The 
average communication bits per round are at most 
$d(M\lceil\log_2[(\frac{\sqrt{n}dT^2}{M})^{1/2}+1]\rceil+
\lceil\log_2[(\sqrt{n}dT^2)^{1/2}+1]\rceil)+(M+1)(d+32)$.

%\mz{write as remarks? Using Stirling's formula, we can improve the average 
%bits 
%per round from 
%$d(M\lceil\log_2(\frac{d\sqrt{n}T^2}{M}+1)\rceil+\lceil\log_2(d\sqrt{n}T^2+1))\rceil+(M+1)(d+32)$
% to 
%$d(M\lceil\log_2(\frac{d\sqrt{n}T^2}{e^2M})\rceil+\lceil\log_2(\frac{d\sqrt{n}T^2}{e^2}))\rceil+(M+1)(2d+32)$
% approximately.}

%Similar to the stochastic case, the key part  of our analysis is to  bound $\| 
%\nabla 
%f(x_t) - \bar{g}_t\|$, which is addressed in 
%\cref{lem:finite_variance_reduction} in \cref{app:var_reduction_finite}. Also 
%since finite-sum optimization can be regarded as a special case 
%of stochastic optimization, the recursive inequality for 
%$\expect[f(x_{t})] - f(x^*)$ can be derived directly 
%from the proof of \cref{thm:distributed}. Combining these two ingredients, 
%\cref{thm:finite_convex} can be derived. 


\subsection{Non-convex Optimization}
\cref{alg:finite_dist_fw} can also be applied to the non-convex setting with a 
slight change in
parameters. We first make a standard assumption on 
the component functions. 

\begin{assump}
	\label{assump_on_f_i}
	Functions $f_{m,i}$ are $L$-smooth on $\constraint$ and bounded, i.e.,  
	$\sup_{x \in 
		\constraint}|f_i(x)| \leq M_0$. 
\end{assump}

%\mz{$x_o \in \constraint$}
%Here we also use the Frank-Wolfe Gap $\mathcal{G}(x)$ to measure the 
%convergence.

%Then we can combine \cref{lem:finite_variance_reduction} and 
%\cref{lem:finite_distributed_nonconvex} to get the theoretical guarantees for 
%non-convex optimization.
\begin{mdframed}
	\begin{theorem}[Proof in 
	\cref{app:thm_quantized_finite_distributed_nonconvex}]
		\label{thm:quantized_finite_distributed_nonconvex}
		Under \cref{assump_on_K,assump_on_f_i}, and $\sup_{x 
			\in \constraint}\|\nabla 
		f_{m,i}(x)\|_\infty \leq G_\infty, \forall\ m \in [M], i 
		\in [n]$, if we set $\eta_t = T^{-1/2}, 
		p=\sqrt{n}, S=\sqrt{n}$, and 
		apply  $s_{1,t}=(2^{z_{1,t}}-1)$-\mscheme $\phi_{1,t}$ and  
		$s_{2,t}=(2^{z_{2,t}}-1)$-\mscheme $\phi_{2,t}$ as $\Phi_{1,t}, 
		\Phi_{2,t}$ in \cref{alg:finite_dist_fw}, where 
		$z_{1,t}=z_1=\lceil 
		\log_2[(\frac{4\sqrt{n}dT}{M})^{1/2}+1] \rceil, z_{2,t}=z_2=\lceil 
		\log_2[(4\sqrt{n}dT)^{1/2}+1] \rceil$, then the output $x_o \in 
		\constraint$ of \cref{alg:finite_dist_fw}  satisfies
		\begin{equation*}
		\expect[\mathcal{G}(x_o)] \leq 
		\frac{2M_0+D\sqrt{L^2D^2+2G_\infty^2}+\frac{LD^2}{2}}{\sqrt{T}}.
		\end{equation*}
		
		%	Moreover, the average communication bits per round are 
		%	$d(Mz_1+z_2)+(M+1)(d+32)$. The LO complexity is $O(1/\epsilon^2)$, 
		%and 
		%the 
		%	IFO complexity is $O(\sqrt{n}/\epsilon^2)$.
	\end{theorem}
\end{mdframed}

\cref{thm:quantized_finite_distributed_nonconvex} shows that for 
non-convex minimization, if we adopt the recommended quantization schemes, then 
\cref{alg:finite_dist_fw} can find an $\epsilon$-first order stationary point 
with at most 
$\mathcal{O}(1/\epsilon^2)$ rounds, \emph{i.e.}, the 
LO complexity is $\mathcal{O}(1/\epsilon^2)$. Also, the total IFO complexity is 
$[Mn+(p-1)\cdot M\cdot S\cdot 2]\cdot \frac{T}{p}= 
\mathcal{O}(\sqrt{n}/\epsilon^2)$. The average communication bits per round 
are $d(M\lceil \log_2[(\frac{4\sqrt{n}dT}{M})^{1/2}+1] 
\rceil+\lceil \log_2[(4\sqrt{n}dT)^{1/2}+1] \rceil)+(M+1)(d+32)$.  


%\mz{$\Phi$ to $\Phi_t$}
%\mz{$x_o \in \constraint$}

%Consider ${g}_t^m$ as the stochastic gradient evaluated by worker $m$ and sent 
%to the master, and $\tilde{g}_t^m$ as the stochastic gradient received by 
%worker $m$ at time $t$. Then, the variance of the stochastic gradient 
%$\tilde{g}_t^m$ can be decomposed into
%%%
%\begin{align}
%    \mathbb{E}[\|\tilde{g}_t^m -\nabla f_{i}(x_t) \|^2\mid {g}_t^m] 
%    &=   \mathbb{E}[\|\tilde{g}_t^m -{g}_t^m \|^2\mid {g}_t^m] +   
%\mathbb{E}[\|{g}_t^m -\nabla f_{i}(x_t) \|^2\mid {g}_t^m] \nonumber\\
%    &=   \mathbb{E}[\|\tilde{g}_t^m -{g}_t^m \|^2\mid {g}_t^m] +   
%\mathbb{E}[\|{g}_t^m -\nabla f_{i}(x_t) \|^2]
%\end{align}

%Using the result from QSGD we know if we have $b$ bits and $s=2^b$ levels of 
%quantization then 
